Learning and Optimization of Implicit Negative Feedback for Industrial Short-video Recommender System

Short-video recommendation is one of the most important recommendation applications in today's industrial information systems. Compared with other recommendation tasks, the enormous amount of feedback is the most typical characteristic. Specifically, in short-video recommendation, the easiest-to-collect user feedback is the skipping behavior, which leads to two critical challenges for the recommendation model. First, the skipping behavior reflects implicit user preferences, and thus, it is challenging for interest extraction. Second, this kind of special feedback involves multiple objectives, such as total watching time and skipping rate, which is also very challenging. In this paper, we present our industrial solution in Kuaishou, which serves billion-level users every day. Specifically, we deploy a feedback-aware encoding module that extracts user preferences, taking the impact of context into consideration. We further design a multi-objective prediction module which well distinguishes the relation and differences among different model objectives in the short-video recommendation. We conduct extensive online A/B tests, along with detailed and careful analysis, which verify the effectiveness of our solution.

==> 6.conclusion.tex <==
\section{Conclusion and Future Work}\label{sec::conclusion}

In this paper, we present the deployed solution for utilizing implicit negative feedback, which is far easier to collect than other behaviors, in the short-video recommendation engine of Kuaishou.
Our solution well combines context-aware feedback learning and multi-objective prediction/optimization, well addressing the two corresponding critical challenges.
The sufficient evaluation through billion-level users' A/B testing demonstrates the effectiveness of the proposed solution.
As for future work, we plan to further combine the sequential modeling into negative feedback learning, further improving preference learning.

\begin{acks}
This work is partially supported by the National Key Research and Development Program of China under 2022YFB3104702, and the National Natural Science Foundation of China under 62272262, 61972223, U1936217, and U20B2060. This work is also supported by Kuaishou.
\end{acks}

==> 7.append.tex <==
\section{APPENDIX FOR REPRODUCIBILITY}
\subsection{Datasets and Evaluation Setting}\label{sec::datasets_info}
We collect two large-scale user consumption data from \textbf{Meituan APP} in the two cities of China (Beijing and Shanghai), from Jan. 1st to Mar. 1st, 2021 (60 days). 
According to the business logic of Meituan,
there are 13 locations and 96 time-slots (dividing a day into 48 time-slots for weekends and weekdays) in the collected datasets.
We only have 19 known intents among a small amount of data ($~17.4\%$), and most of the user consumption behaviors lack intent labels.
To evaluate the model performance in the offline intent discovery task, we split the first 48 days' data as the training set, the following 6 days' data as validation set, and the last 6 days' data as testing set. 
Specifically, we select the first 10 intents as known intents and treat the remaining 9 intents as unknown ones (10 known + 9 unknown intents). We regard the data with known intents and part of the unknown intents data as training set\footnote{We conduct sampling strategy when obtaining training set to ensure the proportion of known intents data ($~17.4\%$) is consistent with the distribution of the original data.}. For the evaluation, we test all the methods on the remaining unknown intents data to evaluate the performance.


\subsection{Baseline Models}\label{sec::baseline_info}
In this section, we give the detailed descriptions of all
compared methods as follows.\\
\textit{(1) Feature generating methods}:
\begin{itemize}[leftmargin=*]
    \item \textbf{DeepFM}~\cite{deepfm} combines the FM and deep neural networks to capture the feature interactions. We concatenate the user ID, location ID, time-slot ID, and category ID as input.
    
    \item \textbf{LightGCN}~\cite{he2020lightgcn} is the state-of-the-art GCN model for recommendation. We adopt it to our task by construct a graph with 6 types of edges among the four types of  nodes (\textit{i.e.}, user, location, time and category). We add the learned node embeddings for each record as the intent feature.
    
    \item \textbf{HAN}~\cite{HAN} is a general state-of-the-art heterogeneous graph learning method. We adapt it to the graph with four types of nodes (user, location, time, and category) by designing three types of meta-path (\textit{user-location, user-time, user-category}) to represent user's preferences on distinct aspects.
\end{itemize}

We combine those feature generating baselines with K-means~\cite{kmeans} to obtain \textbf{DeepFM-KM}, \textbf{LightGCN-KM}, and \textbf{HAN-KM} for the
consumption intent discovery task in Meituan.\\
\textit{(2) Deep clustering methods}:
\begin{itemize}[leftmargin=*]
    \item \textbf{CDAC+}~\cite{CDAC+} refines the cluster results by forcing the model to learn from the high confidence assignments for intent discovery.
    
    \item \textbf{DeepAligned}~\cite{deepaligned} is the SOTA method for intent discovery in dialogue systems, which proposes an alignment
    strategy to tackle the label inconsistency problem during clustering
    assignments.
    
    \item \textbf{DTC}~\cite{DTC} extends the Deep Embedded Clustering to a  transfer learning setting by introducing the temporal ensemble and consistency for the new category discovery.
    
    \item \textbf{RankStat}~\cite{rankstat} is the SOTA method for the new category discovery, which uses pairwise labeling and rank statistics to transfer knowledge of the labeled classes to the unlabeled data.
\end{itemize}

We replace the feature encoder of the deep clustering methods with HAN~\cite{HAN} (the encoder with best performance) to obtain \textbf{HAN-CDAC+}, \textbf{HAN-DeepAligned}, \textbf{HAN-DTC}, and \textbf{HAN-RankStat} for the consumption intent discovery task in Meituan.


\subsection{Metrics}
\subsubsection{Metrics for the intent discovery task} Following~\cite{deepaligned}, we adopt three widely used clustering metrics, \textbf{ACC} (Accuracy), \textbf{ARI} (Adjusted Rand Index), and \textbf{NMI} (Normalized Mutual Information), to evaluate the performance of the intent discovery task. 
Note that we first match the predicted intent label and the ground-truth label with the Hungarian algorithm\cite{kuhn1955hungarian} when calculating \textbf{ACC}.

\subsubsection{Metrics for the recommendation task}
Following~\cite{he2020lightgcn,joglekar2020neural}, we use two widely used ranking-based metrics, \textbf{Recall@K} and \textbf{NDCG@K} (we set K as 10 by following~\cite{he2020lightgcn,lidisenhcn}), to evaluate the performance of the recommendation task. 

\subsection{Implementation Details}
\label{sec::Imp}
\subsubsection{Efficient Implementation for Large-scale Industrial Datasets}
Given that the user number is huge in large scale datasets from Meituan, for all of the graph-based encoders (\textit{i.e.}, LightGCN, HAN, and the dual-hypergraphs in our AutoIntent), the propagation on the graph is very time-consuming. 
Inspired by GraphSAGE~\cite{hamilton2017inductive}, instead of training node embedding with its all neighbors, we propose to sample local neighborhoods for each node and update its embedding by aggregating features from its local neighborhoods.
Specifically, we conduct the sample strategy in a mini-batch manner. Given B nodes in a mini-batch and the sample number is N, the cost of message passing is $\mathcal{O}(BN)$, which is more efficient and only related to the mini-batch size and sample number. Hence, with the above sample strategy, the graph-based methods can be used in large-scale industrial datasets.
Following GraphSAGE~\cite{hamilton2017inductive}, we set the sample number $N$ as 25 in our AutoIntent model for the two datasets from Meituan.


\subsubsection{Hyper-parameter Settings}
For all the models, the embedding size and hidden state size are set as 64, the batch size is set to 2048. We optimize all the methods with Adam~\cite{kingma2014adam} optimizer, which initializes learning rate as 0.001 and will decay it by 0.1 after every three epochs. We also utilize early stopping to detect over-fitting, and the training process will be stopped if ACC on the validation set does not increase for five epochs.
For the baseline methods, we initialize the hyper-parameters as the original papers and carefully tune them to get optimal performance.
For AutoIntent, we set the initial number of all intents $K'$  as $3K^k$ when estimating intent number. We further study the impact of other essential hyper-parameters (the layer number of dual hypergraphs in intent encoders $L$ and the independent coefficient $\lambda$) in section~\ref{sec::hyper_para}.
\textit{{For all methods, we run ten times with the same partition
and report the average results}}.



\subsection{Additional Ablation Study}\label{sec::add_ablation}
In this section, we further provide the additional ablation study of \textit{Denoised Similarity Methods} and \textit{Training Scheme}.

\begin{table}[t]
	\small
	\setlength{\abovecaptionskip}{0.cm}
	\setlength{\belowcaptionskip}{-0.cm}
	\caption{Ablation Study of the Denoised Similarity Methods.}
	\label{tab::Ablation_ds}
	\centering
	\setlength\tabcolsep{5pt}
	\scalebox{0.9}{
		\begin{tabular}{c|ccc|ccc}
			\toprule[1pt]
			\multicolumn{1}{c|}{\bf Dataset} & \multicolumn{3}{c|}{\bf Beijing} &  \multicolumn{3}{c}{\bf Shanghai} \\ 
			\hline
			\bf Model Variants  & \bf ACC        & \bf ARI   &    \bf NMI  
		     &    \bf ACC        & \bf ARI   &    \bf NMI 
			\\ \hline
			RS    & 78.35  &     49.71    & 41.87  & 76.20       
			& 45.54      & 50.56 \\ 
			Cosine    & 78.88  &     50.09    & 42.08       & 76.28       
			&     45.62      & 50.67     \\ 
			HPFFT    & 72.63  &     31.77    & 31.10       & 76.25   &     45.34      & 50.61     \\ 
			BPFFFT    & 75.99  &     41.96    & 36.53       & 76.79   &     49.75      & 50.73     \\ 
			\bf LPFFT     & \bf81.07  &     \bf57.34   &  \bf46.81        & \bf77.39      
			&  \bf50.27      & \bf53.35 \\ 
			\bottomrule[1pt]
	\end{tabular}}
	\vspace{0.4cm}
\end{table}

\vspace{0.2cm}
\subsubsection{Ablation Study of Denoised Similarity Methods}
We combine the \textit{Low-Pass Fast Fourier Transform} (LPFFT) and Cosine similarity to calculate the pairwise pseudo labels in eq.~\eqref{eqn::LPFFT}.
In this section, we further compare the LPFFT with other alternative denoised similarity methods, \textit{i.e.}, ranking statistics proposed in~\cite{rankstat} (RS), cosine similarity without denoising (Cosine), High-Pass Fast Fourier Transform (HPFFT), Band-Pass Fast Fourier Transform (BPFFT). From the results in Table~\ref{tab::Ablation_ds}, the denoised methods (RS, LPFFT) achieve the better performance. Among the methods with filter algorithms, HPFFT achieves the worst performance while LPFFT achieves the best, which verifies that the higher-frequency signals are more likely to be noisy and filtering out them contributes to better performance.


\begin{table}[t]
	\small
	\setlength{\abovecaptionskip}{0.cm}
	\setlength{\belowcaptionskip}{-0.cm}
	\caption{Ablation Study of the training scheme.}
	\label{tab::Ablation_train}
	\centering
	\setlength\tabcolsep{5pt}
	\scalebox{0.9}{
		\begin{tabular}{c|ccc|ccc}
			\toprule[1pt]
			\multicolumn{1}{c|}{\bf Dataset} & \multicolumn{3}{c|}{\bf Beijing} &  \multicolumn{3}{c}{\bf Shanghai} \\ 
			\hline
			\bf Model Variants  & \bf ACC        & \bf ARI   &    \bf NMI  
		     &    \bf ACC        & \bf ARI   &    \bf NMI 
			\\ \hline
			w/o PRE    & 77.96  &     53.43    & 44.25      & 74.71       
			&     47.49      & 51.18  \\ 
			w/o FT    & 80.15  &     56.98    & 45.52       & 76.81   &     49.75      & 52.84     \\ 
			w/o JL    & 80.42  &     57.16    & 46.58       & 76.94   &     49.91      & 52.95     \\ 
			\hline
			\bf AutoIntent     & \bf81.07  &     \bf57.34   &  \bf46.81        & \bf77.39      
			&  \bf50.27      & \bf53.35 \\ 
			\bottomrule[1pt]
	\end{tabular}}
\end{table}


\begin{figure}[t]
	\centering
	\subfloat[\texttt{Snack}]{\includegraphics[width=4.4cm]{figs/intent1.pdf}}
	\subfloat[\texttt{Doing Exercise}]{\includegraphics[width=4.4cm]{figs/intent2.pdf}}
	\setlength{\abovecaptionskip}{0.cm}
	\setlength{\belowcaptionskip}{0.cm}
	\caption{The attention distributions of each disentangled aspects for two intents (\texttt{Snack} and \texttt{Doing Exercise}).} 
	\label{fig::case_study}
\end{figure}

\subsubsection{Ablation Study of Training Scheme}
As for the training scheme of AutoIntent, we first pre-train the disentangled intent encoders with both the labeled and unlabeled data (don't use intent label). Then, we fine-tune the classifier for known intents on the labeled data. Finally, we transfer the knowledge form the known intents to unknown ones with the peseudo-label enhanced joint learning. To verify the effectiveness of the each step in training scheme, we compare the performance of model variants that without pre-training (w/o PRE), without fine-tuning (w/o FT), without
peseudo-label enhanced joint learning (w/o JL) and AutoIntent.
From the results in Table~\ref{tab::Ablation_train}, we can observe that removing any training step will cause significant performance drop. Among them, removing the pre-training of disentangled intent encoders causes a dramatic drop , which verifies that the pre-training without intent label indeed captures the user preference without bias and can generate the transferable intent features.

\subsection{Case Study}
We assume that user consumption behaviors are related to multiple aspects (\textit{i.e.}, location, time, and category). Hence, we design disentangled intent encoders to obtain the intent feature in each aspect and further conduct intent discovery in a disentangled manner.
To verify the effectiveness of the disentangled setting in the user consumption intent discovery task, we select two kinds of discovered new intents (\textit{i.e.}, \texttt{snack} and \texttt{doing exercise}) for case study.
Specifically, we conduct the attention distribution analysis with a box plot for the attention weights calculated from the disentangled intent features in Eq.~\eqref{eqn::predict}.
From the results in Figure~\ref{fig::case_study}, we can observe that the attention distributes in different intents are quite different.
For the intent \texttt{snack}, the attention values in the category aspect are larger than other aspects, which means that the consumption intent \texttt{snack} is more related to users' intrinsic preference, such as taste and brand.
For the intent \texttt{doing exercise}, the attention values in location and category aspects are larger than the time aspect, which means the user who wants to do exercise can be more likely to be influenced by the location factor (where he/she is) and intrinsic preference (which sport he/she likes).
In short, the results of the case study further verify the effectiveness of the disentangled setting in our AutoIntent model.



